AI for IT Operations (AIOps) on Cloud Platforms: Reviews, Opportunities and Challenges

Artificial Intelligence for IT operations (AIOps) aims to combine the power of AI with the big data generated by IT Operations processes, particularly in cloud infrastructures, to provide actionable insights with the primary goal of maximizing availability. There are a wide variety of problems to address, and multiple use-cases, where AI capabilities can be leveraged to enhance operational efficiency. Here we provide a review of the AIOps vision, trends challenges and opportunities, specifically focusing on the underlying AI techniques. We discuss in depth the key types of data emitted by IT Operations activities, the scale and challenges in analyzing them, and where they can be helpful. We categorize the key AIOps tasks as - incident detection, failure prediction, root cause analysis and automated actions. We discuss the problem formulation for each task, and then present a taxonomy of techniques to solve these problems. We also identify relatively under explored topics, especially those that could significantly benefit from advances in AI literature. We also provide insights into the trends in this field, and what are the key investment opportunities.

==> apendix_comparison.tex <==
[In this section we will discuss existing literatures about a variety of topics in AIOps domain, as well as clarify common questions about similarity and difference between AIOps and other related areas.]  

AIOps is a new subdomain of IT operations and it is easy to mix-use with several other concepts such as DevOps, MLOps, etc. This section we try to explain and clarify the overlaps and difference of these IT operation subdomains.

\subsubsection{AIOps vs. DevOps}
DevOps is a model that combines processes of development and operations, in order to deliver software products more efficient than traditional software development processes, where development and operation teams are usually separated. DevOps model enables fast speed development and continuous delivery, meanwhile DevOps with well-designed continuous integration and continuous deliver (CI/CD) infrastructures improves the reliability and security of the software products. DevOps adopts “agile development” methodologies to achieve the above goals, including Scrum, Kanban, Sprints, etc.

AIOps, working under the similar DevOps development models, aims to apply AI and ML techniques to achieve highly efficient development and fully-automated operations. AIOps will reduce human intervention during the entire DevOps lifecycle so DevOps team can focus more on developing features rather than operational related works such as monitoring dashboards, resolving repeated incidents, manually scaling resources, etc.


\subsubsection{AIOps vs. MLOps}
MLOps [AIOps vs. MLOps (https://neptune.ai/blog/mlops-vs-aiops-differences)] represents machine learning operations, which is also an emerging subdomain of IT operations. More and more machine learning solutions are integrated into the software product, such as search engines, recommendation systems, vision and language related products. The backend infrastructure of these services and applications are different than traditional software because they need to manage very complex ML components. MLOps focuses on developing tools and infrastructures to integrating these ML components into the product pipelines. 

That is to say, AIOps is developing AI solutions to improve DevOps pipelines, while MLOps is developing special DevOps pipelines that can support ML services. 

% \section{Survey Methods: Contribution of this article}
% This article is to provide a holistic top-down view of AIOps research and industry. Also with the research we would like to provide foresee of the AIOps trends in the next few years to decades. 

% We first discuss the common problems in industry that can be categorized into AIOps domain. Then we summarizes the existing work of AIOps domain that covers different problems. Lastly, we share our learnings and knowledge about the emerging challenges and future trend in AIOps domain.

==> tables/trace_table.tex <==
% Abandoned
\begin{table*}[hp]
\centering
\caption{Example of trace record logs}
\begin{tabular}{|c|c|c| c| } \hline
 timestamp &  span\_id & message & service  \\ \hline
 1519747202149 & 45f57bb270cb & message-1 & service-A \\ \hline
 1519747202159 & 752877e67bc4 & message-2 & service-A \\ \hline
 1519747202169 & 2997300648a4 & message-3 & service-B \\ \hline
\end{tabular}
\label{table:trace_example}
\end{table*}
